Viscous Destabilization for Large Shocks of Conservation Laws

The recent theory of $a-$contraction with shifts provides $L^2$-stability for shock waves of $1-$D hyperbolic systems of conservation laws. The theory has been established at the inviscid level uniformly in the shock amplitude, and at the viscous level for small shocks. In this work, we investigate whether the $a-$contraction property holds uniformly in the shock amplitude for some specific systems with viscosity. We show that in some cases, the $a-$contraction fails for sufficiently large shocks. This showcases a "viscous destabilization" effect in the sense that the $a$-contraction property is verified for the inviscid model, but can fail for the viscous one. This also shows that the $a$-contraction property, even among small perturbations, is stronger than the classical notion of nonlinear stability, which is known to hold regardless of shock amplitude for viscous scalar conservation laws.

==> notes.tex <==
probably cite moon jin paper on using different entropies for fluxes with exponential growth

\begin{equation}\label{inviscid}
\begin{cases}
u_t+[f(u)]_x=0 & (x,t) \in \mathbb{R} \times (0,\infty) \\
u(x,0)=U_0(x) 
\end{cases}
\end{equation}
\par The inviscid model also admits shock solutions that satisfy the conservation law in the sense of distributions:
\begin{equation}\label{inviscidshock}
v(x,t)=
\begin{cases}
u_- & x < \sigma t \\
u_+ & x > \sigma t 
\end{cases}
\end{equation}
The shock speed $\sigma$ is also calculated the same way via the Rankine-Hugoniot condition.

\par In regards to the inviscid case, it is well known that solutions to \eqref{inviscid} form an $L^1$-contractive semigroup \cite{MR0267257}. For initial data with sufficiently small total variation, the $L^1$-semigroup structure holds for systems of conservation laws \cite{MR1723032}. Regarding the study of the inviscid limit, the $L^1$-based framework was used to prove that for initial data with sufficiently small variation, the solutions to the viscous problem \eqref{viscous} converge to the solution of the Cauchy problem for the inviscid problem \eqref{inviscid} \cite{MR2150387}. 

$\tilde{v}$ is a monotone function, so we may make the change of variable $y=\tilde{v}(\xi)$ and define:
\begin{align*}
    w(y,t)=u^{-X}(\tilde{v}^{-1}(y),t)-y \\
    g(y,t)=h^{-X}(\tilde{v}^{-1}(y),t)-\tilde{h}(\tilde{v}^{-1}(y))
\end{align*}

\begin{proposition}\label{localexistence}
Let $U_0 \in W^{1,\infty}(\mathbb{R})$. Then, there exists a solution $u$ to \eqref{viscous} on $\mathbb{R} \times \R^+$ such that the weak-$*$ limit of $\partial_x u(t,\cdot)$ as $t$ goes to $0$ is $\partial_xU_0$, and $u(t,\cdot)$ converges to $U_0$ in $L^{\infty}$. Furthermore, for every $t \in \R^+$ $$\|U(\cdot,t)\|_{\infty} \leq \|U_0\|_{\infty}$$
\end{proposition}
\begin{proof}
For $T \in \R^+$ fixed, consider the Banach space 
\begin{align*}
    B_T=\lbrace u \in L^{\infty}([0,T];W^{1,\infty}(\mathbb{R})) | u \in C^0((0,T],W^{1,\infty}(\mathbb{R})) \rbrace
\end{align*}
equipped with norm:
\[
||u||_B=\max_{0 \leq t \leq T}||u(t)||_{W^{1,\infty}}
\]
Consider the operator $S$ on $B$, defined as:
\[
\Gamma(u)(u)=e^{t \partial^2_x}U_0-\int_0^t\partial_x\left( e^{(t-s)\partial^2_x}(A(u(s))) \right)ds
\]
%(here, $e^{\Delta t}(u)$ for $u \in L^{\infty}(\R)$ is the convolution with the heat kernel of $u$).\\
Let $B_T(0,R)$ be the unit ball of radius $R$ in $B_T$. We will show that for $T,R$ chosen adequately, $S$ maps $B_T(0,R)$ to $B_T(0,R)$. Let $||u||_B \leq R$.
\[
||\Gamma(u(t))||_\infty \leq ||e^{t\partial^2_x}U_0||_\infty+||\int_0^t\partial_xe^{(t-s)\partial^2_x}*A(u(s))ds||_\infty
\]
For the first, we may use $L^1$ bounds on the heat kernel and Young's convolution inequality:
\[
||e^{t\partial^2_x}U_0||_\infty \leq ||U_0||_\infty
\]
For the integral term in $s$, we use $L^1$ bounds on the derivative of the heat kernel and Young's convolution inequality:
\[
||\int_0^t\partial_xe^{(t-s)\partial^2_x}\left(A(u(s))\right)ds||_\infty \leq C(A) \int_0^t\frac{1}{\sqrt{t-s}}||u(s)||_\infty ds
\]
Similarly, we obtain for the spatial derivative of $S(u)$ (with, this time, a constant depending on $A$ and $R$)
\begin{align*}
    \|\partial_x\Gamma(u)\| \leq \|\partial_xU_0\|_{\infty} + C(A,R) \int_{0}^t\dfrac{1}{\sqrt{t-s}}\|\partial_xu(s,\cdot)\|_{\infty}ds
\end{align*}
(Here notice that for $v \in W^{1,\infty}$ $$\partial_x(e^{t\partial^2_x}(v))=e^{t\partial^2_x}(\partial_xv)$$
where $e^{t\partial^2_x}(\partial_xv)$ is understood as usual in the sense of the convolution against the heat kernel.) \\
Let $R=1+2||U_0||_{W^{1,\infty}}$. Then, for $T$ positive small enough, $S$ maps $B_T(0,R)$ into $B_T(0,R)$. Finally, we show that $S$ is a contraction on $B_T(0,R)$ (after possibly shrinking $T$ to some smaller positive number)
\[
\|\Gamma(u(t))-\Gamma(v(t))\|_\infty \leq C(A) \int_0^t\frac{1}{\sqrt{t-s}}\|u(s)-v(s)\|_\infty ds \leq C(A)\sqrt{T}\|u-s\|_B
\]
We see that $\Gamma$ is a contraction for $T$ sufficiently small. Thus, there exists a fixed point of the equation, which grants a smooth solution to \eqref{viscous} up to time $T$. The uniqueness comes from the fixed point theorem (applied possibly on a bigger ball and smaller time interval) combined with a standard bootstrap argument. \\
By existence and uniqueness of a local in time solution for any $W^{1,\infty}$ data initial, there exists a unique maximal solution for any given initial data. Now, fix an initial data $U_0$, with the associated solution defined on $[0,T)$ for $T \in (0,\infty ]$, and if $T<\infty$ then $$\limsup_{t \rightarrow T} \|u(\cdot,t)\|_{W^{1,\infty}}=\infty$$ \\
The smoothness of the solution on $(0,T) \times \R$ comes from parabolic regularization and induction. One shows that if for some $k \in \mathbb{N} \cup \lbrace 0 \rbrace$ $u \in C^0([T',T),W^{k,\infty})$ for some $0 < T' < T$ such that the solution exists up to time $T$ at least, then $u \in C^0((T',T),W^{k+1,\infty}(\R))$. Hence, by induction, for every $k \in \mathbb{N}$, $u \in C^0((0,T),W^{k,\infty}(\R)$. \\
Hence, as $\partial_tu=-\partial_x(A(u))+\partial^2_xu$ in the distributional sense, an other induction shows that $u$ is smooth on $(0,T) \times \R$.\\
By the maximum principle, $\|u(t)\|_{\infty}$ remains uniformly bounded in $\|u_0\|_{\infty}$ on the interval of existence of $u$.\\
Finally, the global existence is obtained by a Gronwall inequality combined with a bootstrap argument. Indeed, with $$\eta(t):=\sup_{0 \leq s \leq t}\|\partial_xu(s)\|_{\infty}$$
First, notice that $\eta$ is continuous on $[0,T)$ (one can check that it is continuous at $0$ through the Duhamel formula and the fact that $t \mapsto \|e^{\Delta t}(U_0)\|_{\infty}$ is continuous).\\
Then, as $U$ is uniformly bounded for the $L^{\infty}$ norm there exists $C$ positive depending only on $\|u_0\|_{\infty}$ such that for any $0 \leq t < T$ $$\eta(t)\leq \eta(0) + \int_{0}^t\frac{C\eta(s)}{\sqrt{t-s}}ds$$
Hence for any $t \leq \tau:=\frac{1}{16C^2}$ $$\eta(t) \leq \eta(0) + 2\sqrt{t}C\eta(t)$$ and so $$\eta(t) \leq 2\eta(0)$$ For $t \geq \tau$,
$$\eta(t) \leq 2\eta(0) + \frac{2C}{\sqrt{\tau}}\int_0^t\eta(s)ds$$
and so we must have $T=\infty$.
\end{proof}
To be able to bound quantitatively a solution with a spatial translate, we need more information. As our initial perturbations will be compactly supported, we can in particular work in the space of exponentially weighted functions
\begin{proposition}\label{expweight}
    Given a viscous shock $S$ with speed $\sigma$ solution of \eqref{viscousshock}, there exists some positive constant $\theta$ such for any $v_0 \in W^{1,\infty}(\R)$ such that $\|v_0e^{\theta|\cdot|}\|_{\infty}<\infty$ and  $\|v_0'e^{\theta|\cdot|}\|_{\infty}<\infty$. Then, the unique global solution $U$ to \ref{viscous} with initial data $S+v_0$ described in \ref{localexistence} satisfies that for every $t$ in $\R_+$, $\|e^{\theta|\cdot|}U(\cdot,t)-S\|_{\infty} < \infty$ and $\|e^{\theta|\cdot|}\left( U(\cdot,t)-S \right)_x \|_{\infty} < \infty$. Furthermore, there exists $\delta$, $T^*$ and $C$ positive such that, if $\|v_0e^{\theta|\cdot|}\|_{\infty}<\delta$ and  $\|v_0'e^{\theta|\cdot|}\|_{\infty}<\delta$ then for any $t \in [0,T^*]$, $\|e^{\theta|\cdot|}U(\cdot,t)-S\|_{\infty} < C\delta$ and $\|e^{\theta|\cdot|}\left( U(\cdot,t)-S \right)_x \|_{\infty} < C$.
\end{proposition}
\begin{proof}
    To prove this proposition, first fix such a shock $S$ connecting $u_-$ to $u_+$ (with $u_->u_+$) and note its speed $\sigma$ and $\theta:=\min(A'(u_-)-\sigma,\sigma-A'(u_+))$.\\
    We will show that if $v_0 \in W^{1,\infty}(\R)$ satisfies 
    $\|v_0e^{\theta|\cdot|}\|_{\infty}<\infty$ and  $\|v_0'e^{\theta|\cdot|}\|_{\infty}<\infty$
    then, for every, for $U(\cdot,t)$ the solution  $t>0$,$\|e^{\theta|\cdot|}U(\cdot,t)-S\|_{\infty} < \infty$ and $\|e^{\theta|\cdot|}\left( U(\cdot,t)-S \right)_x \|_{\infty} < \infty$.\\
    Notice that the set $$B:=\lbrace t \in \R_+ \, | \, \|e^{\theta|\cdot|}U(\cdot,t)-S\|_{\infty} < \infty \; \text{and} \; \|e^{\theta|\cdot|}\left( U(\cdot,t)-S \right)_x \|_{\infty} < \infty \rbrace$$ is closed in $\R_+$ (by the use of a weak-$*$ topology argument). We just need to show that if $t \in B$ then there is $h>0$ such that $[t,t+h] \subset B$. Indeed, we will then have that $B=\R_+$ by a continuity argument.\\
    For that, we will notice that we have the Green's function representation of $e^{t\partial^2_x}$, given by, for every $v \in L^{\infty}(\R)$ $$e^{t\partial^2_x}(v)(x)=\int_{\R}\frac{e^{-\frac{(x-y)^2}{4t}}}{2\sqrt{\pi t}}v(y)dy$$
    Furthermore, we use the Duhamel formulation used in the proof of \ref{localexistence}, for every such $v_0$, the solution $U$ is given as a fixed point on a small time interval of a Duhamel formulation. \\
    That is, starting with the function constant in time $U_0(\cdot,t):=S+v_0$ at every $t$ and defining inductively the sequence $(U_n)_n$ by
    $$U_{n+1}(\cdot,t)-S(\cdot - \sigma t)=e^{t\partial^2_x}(v_0)+\int_0^te^{(t-s)\partial^2_x}\left(\partial_x(A(S(\cdot-\sigma s))-A(U_n(\cdot,s)))\right)ds$$
    Due to form of the heat kernel, there exists $C>0$ such that for every $w_0 \in L^{\infty}_{\theta}(\R):=\lbrace w_0e^{-\theta |\cdot|} \, | \, w_0 \in L^{\infty}(\R) \rbrace$, $$\|e^{t\partial^2_x}(h)\|_{L^{\infty}_{\theta}}\leq C\|h\|_{L^{\infty}_{\theta}}$$
    This allows to show uniform bounds on the $\|\cdot\|_{L^{\infty}_{\theta}}$ norm of $U_n(\cdot,t)-S(-t\sigma)$ and its spatial derivative for every $n \in \mathbb{N}$. In particular, it shows that there exists $C$, $\delta$ and $T$ positive such that for $\|v(\cdot,t)\|_{\infty}$ uniformly bounded on $\R^+$, then, on $[0,T]$, 
    \begin{align*}
        \left\|\int_0^te^{(t-s)\partial^2_x}\left(\partial_x(A(S(\cdot-\sigma s)+v(\cdot,s))-A(S(\cdot-\sigma s)))\right)ds\right\|_{L^{\infty}_{\theta}}& \\
        \leq C\sup_{0 \leq s \leq t}\|v(\cdot,s)\|_{L^{\infty}_{\theta}}\sqrt{t}&
    \end{align*}
    and similarly for the spatial derivative 
    \begin{align*}
        \left\|\int_0^te^{(t-s)\partial^2_x}\left(\partial_x(A'(S(\cdot-\sigma s)+v(\cdot,s))-A'(S(\cdot-\sigma s))S')\right)ds\right\|_{L^{\infty}_{\theta}}& \\
        \leq C\sup_{0 \leq s \leq t}\|v(\cdot,s)\|_{L^{\infty}_{\theta}}\sqrt{t}&
    \end{align*}
    \begin{align*}
        \left\|\int_0^te^{(t-s)\partial^2_x}\left(\partial_x(A'(S(\cdot-\sigma s)+v(\cdot,s))\partial_xv)\right)ds\right\|_{L^{\infty}_{\theta}}& \\
        \leq C\sup_{0 \leq s \leq t}\|\partial_xv(\cdot,s)\|_{L^{\infty}_{\theta}}\sqrt{t}&
    \end{align*}
    As a consequence, for $\|U(\cdot,t)\|_{L^{\infty}}$ bounded fixed, there exists $T$ positive small enough and $M$ positive great enough such that for every $t$ in $[0,T]$ $$\|v(\cdot,t)\|_{L^{\infty}_{\theta}}\leq M\|v_0\|_{L^{\infty}_{\theta}}$$
\end{proof}

Furthermore, as $Y(u_0-S)=0$, there exists $C$ and $T$ positive constants such that for any $t$ in $[0,T]$ and any $n \in \N$ $$|Y(U(S^{-1}\left(\cdot\right)+X_n(t),t)-S)| \leq C$$ and $$|Z(U(S^{-1}\left(\cdot\right)+X_n(t),t)-\cdot)-Z(u_0(S^{-1}(\cdot))-\cdot)| \leq Ct \; .$$ \\
this comes from \ref{expweight} as the $L^{\infty}_{\theta}$ norm of the spatial derivative of $U(\cdot,t)-S$ remains uniformly bounded for small times.\\
Hence, for any $t$ small enough and any $n \in \mathbb{N}$
\[
\frac{d}{dt}\int_\mathbb{R} a(x)|U(x+X_n(t),t)-S(x)|^2dx|_{t=s} \geq \dfrac{c}{2}
\]
and so for $T^*$ small enough, for any $0 \leq t \leq T^*$ and $n \in \mathbb{N}$
\[
\int_\mathbb{R} a(x)|U(x+X_n(t),t)-S(x)|^2dx \geq \dfrac{ct}{2}+\int_\mathbb{R} a(x)|U_0(x)-S(x)|^2dx >\int_\mathbb{R} a(x)|U_0-S(x)|^2dx
\]
We may take the limit in $n$ (utilizing the fact that $||X_n-X||_\infty \to 0$) to obtain for all $t \in (0,T^*]$
\[
\int_\mathbb{R} a(x)|U(x+X(s),s)-S(x)|^2dx > \int_\mathbb{R} a(x)|U_0-S(x)|^2dx 
\]
as desired, using the continuity of the translation in $L^2(\R)$.

Finally, we need a bound on the $L^2$ norm of a translate of the shock $S$, depending only on the $L^\infty$ norm of the translate. Note that while $S$ is not in $L^2$, $S$ minus a translate of itself is.
\begin{lemma}\label{shifttranslate}
Let $S$ solve \eqref{viscousshock}. Let $m \in \mathbb{R}$. Then:
\[
||S(\cdot)-S(\cdot+m)||_2 \leq C \sqrt{|m|}
\]
\end{lemma}
\begin{proof}
We calculate using Fubini's Theorem:
\[
||S(\cdot)-S(\cdot+m)||_2^2 \leq 2||S||_\infty ||S'||_1|m|
\]
Taking the square root gives the result. 
\end{proof}

\leq |\int_\mathbb{R} (a''^{X_n(t)}-a'')(U(t)-S^{X_n(t)})^2dx|+ \\
|\int_\mathbb{R}a''(U(t)-S^{X_n(t)})(U(t)-U(0))dx|+|\int_\mathbb{R} a''(U_0-S^{X_n(t)})(U(t)-U_0)dx|+ \\
|\int_\mathbb{R} a''(U_0-S^{X_n(t)})(S-S^{X_n(t)})dx|+|\int_\mathbb{R}''(U_0-S)(S-S^{X_n(t)})dx| \leq \\
||a'''||_\infty||\dot{X_n}||_\infty t(||U(t)||_\infty+||S||_\infty)^2)+ \\
||a''||_\infty(||U(t)-S||_2+||S-S^{X_n(t)}||_2)(||U(t)-U_0||_2)+ \\
||a''||_\infty(||U_0-U(t)||_2+||U(t)-S||_2+||S-S^{X_n(t)}||_2)(||U_0-U(t)||_2 + \\
||a''||_\infty(||U_0-U(t)||_2+||U(t)-S||_2+||S-S^{X_n(t)}||_2)||S-S^{X_n(t)}||_2+ \\
||a''||_\infty ||U_0-S||_2||S-S^{X_n(t)}||_2
